Nonlocal Neural Tangent Kernels via Parameter-Space Interactions

The Neural Tangent Kernel (NTK) framework has provided deep insights into the training dynamics of neural networks under gradient flow. However, it relies on the assumption that the network is differentiable with respect to its parameters, an assumption that breaks down when considering non-smooth target functions or parameterized models exhibiting non-differentiable behavior. In this work, we propose a Nonlocal Neural Tangent Kernel (NNTK) that replaces the local gradient with a nonlocal interaction-based approximation in parameter space. Nonlocal gradients are known to exist for a wider class of functions than the standard gradient. This allows NTK theory to be extended to nonsmooth functions, stochastic estimators, and broader families of models. We explore both fixed-kernel and attention-based formulations of this nonlocal operator. We illustrate the new formulation with numerical studies.

==> sec1.tex <==

\begin{abstract}
We propose a novel framework for approximating the Nonlocal Neural Tangent Kernel (NTK) using an attention-weighted Monte Carlo (MC) estimator. Our approach extends the classical NTK framework to nonlocal and stochastic variants by interpreting nonlocal gradients as expectations over random perturbations in parameter space. We introduce a learnable attention mechanism over sampled parameter offsets, allowing adaptive control of the NTK contributions during training. The sample count $N$ in the MC approximation is also made learnable, enabling dynamic trade-offs between accuracy and computational cost. We provide theoretical results on consistency and bias-variance trade-offs, and conduct spectral and alignment-based comparisons between our method, standard NTK, and its deterministic and uniformly-sampled nonlocal analogs. Experiments on non-smooth regression tasks such as the sign and sawtooth functions demonstrate the advantages of our approach.
\end{abstract}

\section{Introduction}
The Neural Tangent Kernel (NTK) \cite{jacot2018ntk} has emerged as a powerful tool for analyzing the training dynamics of wide neural networks. However, traditional NTK theory assumes infinitesimal parameter updates and linearized training dynamics, which can fall short in capturing nonlocal behavior of real-world networks. Inspired by nonlocal calculus, we formulate a \textit{Nonlocal NTK} framework based on finite parameter perturbations.

We further propose a stochastic approximation of the Nonlocal NTK using Monte Carlo sampling over random parameter perturbations. To increase flexibility and adaptivity, we introduce an attention-based mechanism that assigns learned weights to each sampled perturbation. This leads to our main contribution: an attention-weighted Monte Carlo estimator of the Nonlocal NTK, with learnable number of samples $N$.

\section{Background and Motivation}
Given a neural network $f(x; \theta)$ with parameters $\theta \in \mathbb{R}^d$, the classical NTK is defined as:
\[
K(x, x') = \nabla_\theta f(x; \theta)^\top \nabla_\theta f(x'; \theta).
\]
The NTK governs the evolution of predictions under gradient flow:
\[
\frac{d}{dt} f(x; \theta_t) = -\sum_{x'} K(x, x') \frac{\partial \mathcal{L}}{\partial f(x')}.
\]
However, the infinitesimal gradient assumption fails to account for finite and nonlocal parameter changes.

\subsection{Nonlocal Gradient Perspective}
Let $\rho_\delta(\theta, \theta')$ be a kernel defining an interaction neighborhood in parameter space. The nonlocal gradient of $f$ at $\theta$ can be expressed as:
\[
\mathcal{D}_\delta f(\theta) := \int \frac{f(\theta') - f(\theta)}{\|\theta' - \theta\|} \rho_\delta(\theta, \theta') d\theta'.
\]
This motivates defining a Nonlocal NTK:
\[
K_\delta(x, x') := \mathbb{E}_{\Delta \sim \rho_\delta} \left[ \frac{f(x; \theta + \Delta) - f(x; \theta)}{\|\Delta\|} \cdot \frac{f(x'; \theta + \Delta) - f(x'; \theta)}{\|\Delta\|} \right].
\]

\section{Monte Carlo Approximation}
We approximate the Nonlocal NTK using $N$ random perturbations $\{\Delta_k\}_{k=1}^N \sim \rho$:
\[
\hat{K}(x, x') = \frac{1}{N} \sum_{k=1}^N \frac{\delta_k(x) \cdot \delta_k(x')}{\|\Delta_k\|^2},
\]
where $\delta_k(x) := f(x; \theta + \Delta_k) - f(x; \theta)$. This estimator can be computed without access to gradients, making it amenable to black-box settings.

\subsection{Attention-Weighted Estimator}
We introduce an attention network $a(\Delta_k; \phi)$ to compute weights $w_k$ satisfying $\sum_k w_k = 1$. The estimator becomes:
\[
\hat{K}_{\text{attn}}(x, x') = \sum_{k=1}^N w_k \cdot \frac{\delta_k(x) \cdot \delta_k(x')}{\|\Delta_k\|^2}.
\]
This allows the model to focus on informative directions in parameter space.

\subsection{Learnable $N$}
We further allow $N$ to be a learnable scalar $\hat{N} \in \mathbb{R}^+$, rounded and clamped during use. This enables dynamic adaptation of computational resources during training.

\section{Theoretical Analysis}

\subsection{Law of Large Numbers}
\textbf{Theorem.} Let $\Delta_1, \dots, \Delta_N$ be i.i.d. samples from $\rho(\Delta)$, and suppose $f$ is Lipschitz in $\theta$. Then:
\[
\hat{K}(x, x') \to K_\delta(x, x') \quad \text{as } N \to \infty \text{ (a.s. and in $L^2$)}.
\]

\textbf{Corollary (Bias and Variance).} The estimator $\hat{K}(x, x')$ has:
\[
\mathbb{E}[\hat{K}(x, x')] = K_\delta(x, x'), \quad \operatorname{Var}[\hat{K}(x, x')] = \frac{\sigma^2}{N}.
\]

\subsection{Online Learning Variant}
In the online setting, we use $N=1$ sample per epoch, accumulating information across training time. This can be interpreted as a stochastic approximation of the full kernel.

\section{Implementation Details}

We implement the method in PyTorch with:
\begin{itemize}
    \item A feedforward network $f(x; \theta)$ for regression.
    \item An attention network $a(\Delta)$ with two-layer MLP.
    \item Automatic detection of GPU.
    \item NTK computed at regular intervals (e.g., every 10 epochs).
\end{itemize}

\section{Experiments}

\subsection{Tasks}
We test on:
\begin{itemize}
    \item \textbf{Sign function}: $f(x) = \text{sign}(x)$
    \item \textbf{Sawtooth function}: $f(x) = 2(x \bmod 1) - 1$
\end{itemize}

\subsection{Variants Compared}
\begin{itemize}
    \item \textbf{Equal MC (Nonlocal)}: Uniform weights $w_k = 1/N$
    \item \textbf{Attention-weighted (Hybrid)}: Learnable weights $w_k$
    \item \textbf{Deterministic Attention}: No sampling, directly assign weights to fixed $\Delta$ values.
\end{itemize}

\subsection{Metrics}
We track:
\begin{itemize}
    \item \textbf{Eigenvalue spectrum} of the NTK matrix.
    \item \textbf{Kernel-target alignment}:
    \[
    \mathcal{A}(K, y) = \frac{y^\top K y}{\|y\|^2 \|K\|_F}
    \]
\end{itemize}

\subsection{Results}
\begin{figure}[h]
    \centering
    \includegraphics[width=0.48\textwidth]{spectrum_sign.png}
    \includegraphics[width=0.48\textwidth]{alignment_sign.png}
    \caption{(Left) NTK spectrum over epochs. (Right) Kernel-target alignment for sign task.}
\end{figure}

We find that attention-weighted variants produce smoother and more stable spectra. The alignment improves faster in hybrid and deterministic attention cases, especially on non-smooth targets.

\section{Discussion}

\paragraph{Adaptive computation.} Learning $N$ allows efficient allocation of resources. In early epochs, small $N$ may suffice; later training may benefit from more samples.

\paragraph{Attention is structure-aware.} The attention network learns to prioritize perturbations that significantly change the network output, mimicking curvature-aware updates.

\paragraph{Relation to NTK theory.} Our method maintains the kernel-based dynamical interpretation, but generalizes the update to nonlocal paths in parameter space.

\section{Conclusion}

We introduced a nonlocal, attention-based variant of the Neural Tangent Kernel using Monte Carlo approximation. By combining learnable sampling strategies with attention mechanisms, we obtain more flexible and expressive kernel dynamics. Future directions include extending to convolutional networks, studying generalization bounds, and applying to continual learning via online NTK updates.




\section*{Nonlocal Gradient Estimator}

Let \( f : \mathbb{R}^d \to \mathbb{R} \) be a locally Lipschitz function, and let \( \rho_\gamma(\theta', \theta) \) be a probability density function supported on a compact set \( \Omega \subset \mathbb{R}^d \), depending on a parameter \( \gamma > 0 \).

The nonlocal gradient operator is defined as:
\[
\mathcal{G}_\gamma f(\theta) := \int_{\Omega} \frac{f(\theta') - f(\theta)}{\theta' - \theta} \rho_\gamma(\theta', \theta) \, d\theta',
\]
where division is interpreted component-wise.

We define the Monte Carlo estimator:
\[
\widehat{\mathcal{G}}^N_\gamma f(\theta) := \frac{1}{N} \sum_{j=1}^N \frac{f(\theta'_j) - f(\theta)}{\theta'_j - \theta},
\]
where \( \theta'_j \sim \rho_\gamma(\cdot \mid \theta) \) are i.i.d.

\section*{Main Result}

\begin{theorem}[Law of Large Numbers for Nonlocal Gradient Estimator]
Let \( f : \mathbb{R}^d \to \mathbb{R} \) be locally Lipschitz, and let \( \rho_\gamma(\cdot, \theta) \) be a probability density with compact support excluding \( \theta \). Assume:
\begin{itemize}
    \item \( \rho_\gamma(\cdot, \theta) \) is supported in a compact set \( \Omega \),
    \item The denominator \( \theta' - \theta \) never vanishes on the support,
    \item The function \( \frac{f(\theta') - f(\theta)}{\theta' - \theta} \) is integrable over \( \rho_\gamma(\cdot \mid \theta) \).
\end{itemize}
Then the estimator \( \widehat{\mathcal{G}}^N_\gamma f(\theta) \) converges:
\[
\widehat{\mathcal{G}}^N_\gamma f(\theta) \xrightarrow{a.s.} \mathcal{G}_\gamma f(\theta) \quad \text{as } N \to \infty,
\]
and also in mean square:
\[
\mathbb{E}\left[ \left\| \widehat{\mathcal{G}}^N_\gamma f(\theta) - \mathcal{G}_\gamma f(\theta) \right\|^2 \right] \to 0 \quad \text{as } N \to \infty.
\]
\end{theorem}

\begin{proof}
Define:
\[
Z_j := \frac{f(\theta'_j) - f(\theta)}{\theta'_j - \theta} \in \mathbb{R}^d.
\]
Each component of \( Z_j \) is bounded due to the Lipschitz continuity of \( f \) and compactness of support. Let:
\[
\mu := \mathbb{E}[Z_j] = \mathcal{G}_\gamma f(\theta).
\]

By the strong law of large numbers (SLLN), the sample mean converges almost surely:
\[
\frac{1}{N} \sum_{j=1}^N Z_j \xrightarrow{a.s.} \mu.
\]

To show convergence in \( L^2 \), we compute:
\[
\mathbb{E}\left[ \left\| \frac{1}{N} \sum_{j=1}^N Z_j - \mu \right\|^2 \right] = \frac{1}{N} \text{Var}[Z_1] \to 0 \quad \text{as } N \to \infty.
\]
\end{proof}

\section*{Bias and Variance Bounds}

\begin{corollary}[Bias and Variance of Estimator]
Assume \( f \) is Lipschitz with constant \( L \), and that \( \theta'_j \sim \rho_\gamma(\cdot \mid \theta) \) with support bounded such that \( \| \theta'_j - \theta \| \geq \delta > 0 \). Then for all \( N \geq 1 \):
\[
\left\| \mathbb{E}\left[ \widehat{\mathcal{G}}^N_\gamma f(\theta) \right] - \mathcal{G}_\gamma f(\theta) \right\| = 0,
\]
i.e., the estimator is unbiased. Moreover, the variance satisfies:
\[
\text{Var}\left[ \widehat{\mathcal{G}}^N_\gamma f(\theta) \right] \leq \frac{C}{N},
\]
for some constant \( C > 0 \) depending on \( L \), \( \gamma \), and the geometry of \( \rho_\gamma \).
\end{corollary}

\begin{proof}
The estimator is unbiased since the expectation of the sample mean equals the true integral:
\[
\mathbb{E}\left[ \widehat{\mathcal{G}}^N_\gamma f(\theta) \right] = \mathcal{G}_\gamma f(\theta).
\]

For variance, since the samples \( Z_j \) are i.i.d., we have:
\[
\text{Var}\left[ \frac{1}{N} \sum_{j=1}^N Z_j \right] = \frac{1}{N} \text{Var}[Z_1].
\]
Due to the boundedness of \( f \) and compact support of \( \rho_\gamma \), \( \text{Var}[Z_1] \leq C \) for some finite constant.
\end{proof}

\section*{Remarks}

\begin{itemize}
    \item This estimator allows differentiation of non-smooth functions where the classical gradient does not exist.
    \item In practice, regularization can be applied to the denominator to avoid numerical instability when \( \theta'_j \approx \theta \).
    \item The estimator enables the use of stochastic sampling techniques in optimization and kernel methods (e.g., NTK).
\end{itemize}


